InfoLossQA: Characterizing and Recovering Information Loss in Text Simplification

Text simplification aims to make technical texts more accessible to laypeople but often results in deletion of information and vagueness. This work proposes InfoLossQA, a framework to characterize and recover simplification-induced information loss in form of question-and-answer (QA) pairs. Building on the theory of Question Under Discussion, the QA pairs are designed to help readers deepen their knowledge of a text. We conduct a range of experiments with this framework. First, we collect a dataset of 1,000 linguist-curated QA pairs derived from 104 LLM simplifications of scientific abstracts of medical studies. Our analyses of this data reveal that information loss occurs frequently, and that the QA pairs give a high-level overview of what information was lost. Second, we devise two methods for this task: end-to-end prompting of open-source and commercial language models, and a natural language inference pipeline. With a novel evaluation framework considering the correctness of QA pairs and their linguistic suitability, our expert evaluation reveals that models struggle to reliably identify information loss and applying similar standards as humans at what constitutes information loss.

==> figures/fig-question-similarity.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=.85\linewidth]{figures/question-similarity-dense}
\caption{Similarity of annotators' questions ($Q$) by whether their evidence spans ($E$) have no/partial/complete overlap. We calculate cosine similarity over sentence embeddings~\cite{Reimers:2019:EMNLP}. Cosine greater 1 is an artifact of the kernel density estimate.}
\label{fig:question-similarity}
\end{figure}


==> figures/tab-results-part2.tex <==
\begin{table*}[t]
\small
\setlength{\tabcolsep}{5pt}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccccc}
\toprule
    & \textbf{Givenness ($Q$)} & \multicolumn{3}{c}{\textbf{Rationale Localization ($R$)}} & \multicolumn{4}{c}{\textbf{Jargon ($A$)}} & \textbf{Standalone ($A$)} & \textbf{Hallu. ($A$)} \\
    \cmidrule(lr){2-2}
    \cmidrule(lr){3-5}
    \cmidrule(lr){6-9}
    \cmidrule(lr){10-10}
    \cmidrule(lr){11-11}
\textbf{Model}  & \% Good & Good & Unrelated$^\downarrow$ & Missing$^\downarrow$ & (++) & (+) & (-)$^\downarrow$ & (-{}-)$^\downarrow$ & \% Good & \% Good \\
\midrule
Mistral-7B & 74.5 & \bfseries 52.0 & 5.9 & \bfseries 42.2 & 21.6 & 9.3 & 13.2 & 55.9 & 84.3 & 96.1 \\
Llama2-70B & 75.2 & 34.5 & 5.3 & 60.2 & 26.2 & 7.8 & 17.5 & 48.5 & 79.6 & 92.2 \\
GPT-4 & \bfseries 82.0 & \bfseries 52.0 & 1.5 & 46.5 & 15.0 & 24.0 & \bfseries 11.0 & 50.0 & \bfseries 90.5 & \bfseries 99.0 \\
NLI Pipeline & 58.3 & 17.6 & \bfseries 0.0 & 82.4 & \bfseries 28.9 & \bfseries 29.9 & 12.7 & \bfseries 28.4 & 86.3 & 98.0 \\
\bottomrule
\end{tabular}
}
\caption{Linguistic suitability of generated QA pairs and hallucinations (hallu).
% We provide the percent of ratings given by two independent annotators over 100 QA pairs per model.
$^\downarrow$ = lower is better.
% The scale for Simplicity indicates if answer contains no jargon (++), answer has jargon but explains it (+), answer has unexplained jargon but simple text explains it (-), or answer has unexplained jargon (-{}-).
}
\label{tab:results-part2}
\end{table*}


==> figures/tab-results-part3.tex <==
\begin{table}[t]
\small
\centering
\begin{tabular}{lrrr}
\toprule
\textbf{Model} & \textbf{Full$^\uparrow$} & \textbf{Partial} & \textbf{No$^\downarrow$} \\
\midrule
Mistral-7B & 14.2 & 4.1 & 81.8 \\
Llama2-70B & 16.2 & 4.4 & 79.3 \\
GPT-4 & \bfseries 28.1 & 3.4 & 68.4 \\
NLI Pipeline & 22.9 & 20.0 & \bfseries 57.2 \\
\bottomrule
\end{tabular}
\caption{Recall (\%) of human-written QA pairs. % across 55 documents (554 QA pairs). A human QA pair can either be fully, partially or not recalled.
}
\label{tab:results-part3}
\end{table}

